RefreshKV: Updating Small KV Cache During Long-form Generation

Generating long sequences of tokens given a long-context input is a very compute-intensive inference scenario for large language models (LLMs). One prominent inference speed-up approach is to construct a smaller key-value (KV) cache, relieving LLMs from computing attention over a long sequence of tokens. While such methods work well to generate short sequences, their performance degrades rapidly for long-form generation. Most KV compression happens once, prematurely removing tokens that can be useful later in the generation. We propose a new inference method, RefreshKV, that flexibly alternates between full context attention and attention over a subset of input tokens during generation. After each full attention step, we update the smaller KV cache based on the attention pattern over the entire input. Applying our method to off-the-shelf LLMs achieves comparable speedup to eviction-based methods while improving performance for various long-form generation tasks. Lastly, we show that continued pretraining with our inference setting brings further gains in performance.

==> figs/algo.tex <==
\begin{figure*}%{r}{0.5\textwidth}
\begin{framed}
\small
\textbf{Input:} LM $M$, Input tokens [$x_{0}, x_{1}, ... x_{L}$], the size of parital KV cache $K$, stride $S$ to refresh partial cache, full KV cache $C_{f}$, partial KV cache $C_{p}$, position in cache $p$ \\
\textbf{Output:} A list of generated tokens $\mathcal{T}$ \\
\textbf{Initialize:} Pre-fill $M$ with [$x_{0}, x_{1}, ... x_{L}$] which computes $C_{f}$; return attention score $\mathbf{a_{L}}$ of the last token $x_{L}$\\

\begin{algorithmic}[1]
\STATE $\mathcal{T} \gets []$, $p \gets 0$
\STATE $C_r \leftarrow \operatorname*{arg\,top-k}_{x \in C_f} \mathbf{a_{L}}$ 

\FOR{$i  \in \{1, 2, \dots, T \}$} 
\IF{$i \mod S == 0$} 
    \IF{$p > 0$}
        \STATE $C_{f}$ = [$C_{f}$, $C_{r}[:-p]]$ \textcolor{blue}{\Comment{$\triangleright$ Update $C_{f}$ with KV cache of previous tokens inferenced with recycled attention}}
    \ENDIF
    \STATE $t, \mathbf{a} = M(C_{f})$  \textcolor{blue}{\Comment{$\triangleright$ Generate token $t$ with $M$ using full cache $C_f$ and return attention scores}} \\ 
    \STATE $\mathcal{T}.\text{append}(t)$\\
    % \STATE $C_{r} = c_{i} \in C_{f}$, if $a_{i}$ \in \mathrm{argTop}k_{$a_{i}$ \in \mathbf{a}}
    \STATE $C_r \leftarrow \operatorname*{arg\,top-k}_{x \in C_f} \mathbf{a}$ \textcolor{blue}{\Comment{$\triangleright$ Recycle KV cache of top $k$ tokens from $C_f$ based on attention scores}} \\
    \STATE $p \gets 1$
\ELSE
\STATE $t = M(C_{r})$ \textcolor{blue}{\Comment{$\triangleright$ Generate token $t$ with $M$ using recycled cache $C_{r}$}} \\ 
\STATE $\mathcal{T}.\text{append}(t)$
\STATE $p += 1$
\STATE $C_{r} = C_{r}[1:]$ \textcolor{blue}{\Comment{$\triangleright$ Remove the token that received the lowest attention score}} \\ 


\ENDIF
% \ENDIF
\ENDFOR

\STATE return $\mathcal{T}$
% \FOR{$i  \in \{1, \dots, |\mathcal{T}| \}$}

% \STATE{ l_{i} = - log\frac{e^{sim(x_{i}, p_{i})}}{e^{sim(x_{i}, p_{i})} + \sum_{j=1}^{B}e^{sim(x_{i}, n_{j})}}}


\end{algorithmic}
\end{framed}
% \vspace{-0.8em}
\caption{Pseudocode for recycled attention. We denote $M(C)$ as performing a forward pass with the language model with cache $C$, which includes updating $C$ with the KV cache for the input tokens. \fy{add notation for updating KV cache of input tokens} }\label{alg:ra}
% \vspace{-2em}
\end{figure*}
